Cohomogeneity one manifolds with quasipositive curvature

In this paper we give a classification of cohomogeneity one manifolds admitting an invariant metric with quasipositive sectional curvature except for two $7$-dimensional families. The main result carries over almost verbatim from the classification results in positive curvature carried out by Verdiani and Grove, Wilking and Ziller. Three main tools used in the positively curved case that we generalized to quasipositively curved cohomogeneity one manifolds are Wilking's Chain Theorem, the classification of positively curved fixed point homogeneous manifolds by Grove and Searle and the Rank Lemma.

==> documents/essential.tex <==
\section{Fixed point homogeneous manifolds}\label{secessential}

In this section we prove that it is enough, to classify the essential actions. The reason for this is Theorem \ref{intro_fp_hom}, which states, that quasipositively curved cohomogeneity one manifolds, that have a subaction that is fixed point homogeneous, are equivariantly diffeomorphic to a rank one symmetric space.\\
%\begin{thm}\label{essential_thm_fixedpt}
%	Let $M$ be a compact quasipositively curved cohomogenity one $G$-manifold, where $G$ is a compact Lie group. Assume there is a subgroup $G^\prime\subset G$, that acts fixed point homogeneous on $M$, then $M$ is equivariantly diffeomorphic to a rank one symmetric space.
%\end{thm}

In positive curvature the result of Theorem \ref{intro_fp_hom} was proven by Grove and Searle in \cite{gs}, without the presence of a surrounding cohomogeneity one action. It relies on the Alexandrov geometry of the orbit space $M^\prime$ of the action. The assumption on fixed point homogeneity implies, that $M^\prime$ has a boundary component corresponding to the fixed point set. By a result of Perelman (cf. \cite{p}), the distance function from the boundary is strictly concave and hence the set at maximal distance to this boundary component is a point. This corresponds to an orbit at maximal distance to the fixed point component. $M$ is now the union of tubular neighbourhoods around the fixed point component and  the orbit at maximal distance glued together at their common boundary. From the uniqueness lemma (\cite{gs}, Lemma 2.5) it follows that $M$ is equivariantly diffeomorphic to a rank one symmetric space. In the case of quasi positive curvature, together with a cohomogeneity one action it is still possible to obtain the orbit at maximal distance to the fixed point set. The remaining proof is handled in the same way as in \cite{gs}.

From now on Let $M$ be a cohomogeneity one $G$-manifold fulfilling the assumptions of Theorem \ref{intro_fp_hom}. We can assume that a normal factor $G^\prime$ of $G$ acts fixed point homogenous. Since the action is assumed to be almost effective $G^\prime$ is contained in one of $K^\pm$, say $K^-$.
Let $\pi^\prime \colon M \to M^\prime$ be the quotient map of the $G^\prime$-action on $M$. Obviously $G^\prime$ acts trivially on $B_-$. Therefore $B_- \subseteq M^{G^\prime}$. Let $F \coloneqq B_-$ and $\bar F \coloneqq \pi^\prime(F)$. Let $d$ denote the orbit metric on $M^\prime$ induced by $\pi^\prime$. Note, that $\bar F$ is a boundary component of $M^\prime$. Let $d_{\bar F} \colon M^\prime \to \bb R$ be the distance function from $\bar F$ in $M^\prime$. The following lemma will be crucial in the proof of Theorem \ref{intro_fp_hom}:
\begin{lem}
	Let $X$ be a cohomogeneity one non negatively curved Alexandrov space with boundary $F$. Assume there is an open set $U \subset X$ which has positive curvature. Then the set $C$ of maximal distance to $F$ consists of a single point.   
\end{lem}
\begin{proof}
%	First suppose there was another fixed point component in $M^{G^\prime}$. By the proof of Theorem 2 in \cite{sy}  $M^\prime$ is isometric to a product $\bar F \times [0,1]$, which forces $\bar F \cong F$ to be a point, since $M$ and hence $M^\prime$ has an open set of positive sectional curvature. So the point of maximal distance is the other boundary point. 
%	Hence we can assume that $F$ is the only fixed point component,  $\bar F$ is the only boundary component of $M^\prime$ and $\dim F > 0$. Note that $M^\prime$ with the orbit distance is an Alexandrov space with non negative curvature. By Theorem 6.1 in \cite{p} the distance function $d_{\bar F}$ is concave. Let $C$ be the set of points in $M^\prime$ of maximal distance from $\bar F$. Since $F$ is the fixed point set of $G^\prime$ and $G^\prime$ is a normal subgroup of $G$, $d_{\bar F}$  coincides with the orbit distance from $F$, which in turn implies, that $C = \pi^\prime(B_+)$. Hence $M^\prime\backslash C$ is actually a smooth manifold with boundary $\bar F$ and $\pi^\prime\vert_{M\backslash B_+}$ is a riemannian submersion. Therefore $M^\prime\backslash C$ hat quasipositive curvature. Note that $G/G^\prime$ acts on $M^\prime$ with cohomogeneity one. 
%
%	We will use the comparison theory for Riccati equations to proof the claim (see for example \cite{eh}). Let $c$ be a normal geodesic from $\bar F$ to $C$ in $M^\prime$. It is induced by a horizontal geodesic in $M$. Since $d_{\bar F}$ is a smooth function on $M^\prime \backslash (\bar F \cup C)$ its hessian induces an $(n-1)$-dimensional Lagrangian family $\Lambda$ of Jacobi fields, which precisely coincide with the action fields of the $G/G^\prime$-action on $M^\prime \backslash C$. The Hessian $A(t)\coloneqq \Hess d_{\bar F}(c(t))$ of $d_{\bar F}$ is a self adjoint operator on $\dot c(t)^\perp$ which solves the Ricatti equation:
%	\begin{align*}
%	A^2(t)+A^\prime(t) + R(t) =0
%	\end{align*}
%	Here $R(t) \coloneqq R( \cdot,\dot c(t))\dot c(t)$. Furthermore the following equation holds
%	\begin{align*}
%	A(t)J(t) = J^\prime(t), \quad \forall \, J \in \Lambda
%	\end{align*}
%	We will now show, that $A(0) = 0$. Since $\bar F$ is the boundary of $M^\prime $ and $G/G^\prime$ acts on $M^\prime$, it is an orbit by this action and induces the tangent space of $\bar F \subset M^\prime$. Therefore let $J_1,J_2 \in \Lambda$
%	\begin{align*}
%	\langle A(0)J_1(0), J_2(0)\rangle = \langle J_1^\prime(0), J_2(0)\rangle = \langle \nabla_{\dot c(0)}J_1(t), J_2(t) \rangle = -\langle \nabla_{J_2(t)}J_1(t), \dot c(0) \rangle = 0
%	\end{align*}
%	The last equation holds since $\bar F$ is totally geodesic. Since $R(t) \ge 0$ and $A(0) =0$ it follows by standard Ricatti comparison, that $A(t) \le 0$, because $B \equiv 0$ solves the Ricatti equation for $R=0$. Note, that this already implies the concavity of $d_{\bar F}$. Furthermore there exists a $t_0$, such that $R(t_0) \ge k >0$. Therefore there exists a $t_1$, such that $A(t) \le l <0$ for all $t>t_1$, since $B(t) = \sqrt k\tan(-\sqrt kt)\cdot \Id$ solves the Ricatti equation for $R = k \cdot \Id$ and $B(0) =0$ and $C(t) = \frac{l}{tl+1} \le l <0$ solves the equation for $R=0$ and $C(0) = l$. Hence $d_{\bar F}$ is actually strongly concave on compact segments of geodesics, which start and end at distance greater that $t_1$ from $\bar F$. Since every geodesic in $C$ can be approximated by geodesics in $M^\prime\backslash C$ the claim follows.
 We will use the partial flat strip property by Shioya and Yamaguchi (see \cite{ShiYa} Prop. 9.10 and \cite{RoWa22} Lemma 1.4). It states the following. Let $X_t \coloneqq \lbrace x \in X \vert d_F(x) \ge t \rbrace$. Furthermore let $c \colon \lbrack 0, 1 \rbrack \to C$ be a geodesic and $\gamma_0$ a shortest geodesic from $c(0)$ to $\partial X_t$ perpendicular to $C$. Then there exists a minimal geodesic $\gamma_1$ from $c(1)$ to $\partial X_t$, such that $\gamma_0$, $c$ and $\gamma_1$ bound a totally geodesic flat strip. Since $X$ has a cohomogeneity one action, a flat strip will always intersect some set of positive curvature. Hence $C$ is a point.
\end{proof}
	
	The proof of Theorem \ref{intro_fp_hom} now works in the exact same way as in \cite{gs}.


